Feature Inference Attack on Shapley Values

As a solution concept in cooperative game theory, Shapley value is highly recognized in model interpretability studies and widely adopted by the leading Machine Learning as a Service (MLaaS) providers, such as Google, Microsoft, and IBM. However, as the Shapley value-based model interpretability methods have been thoroughly studied, few researchers consider the privacy risks incurred by Shapley values, despite that interpretability and privacy are two foundations of machine learning (ML) models. In this paper, we investigate the privacy risks of Shapley value-based model interpretability methods using feature inference attacks: reconstructing the private model inputs based on their Shapley value explanations. Specifically, we present two adversaries. The first adversary can reconstruct the private inputs by training an attack model based on an auxiliary dataset and black-box access to the model interpretability services. The second adversary, even without any background knowledge, can successfully reconstruct most of the private features by exploiting the local linear correlations between the model inputs and outputs. We perform the proposed attacks on the leading MLaaS platforms, i.e., Google Cloud, Microsoft Azure, and IBM aix360. The experimental results demonstrate the vulnerability of the state-of-the-art Shapley value-based model interpretability methods used in the leading MLaaS platforms and highlight the significance and necessity of designing privacy-preserving model interpretability methods in future studies. To our best knowledge, this is also the first work that investigates the privacy risks of Shapley values.

==> tex-files/sec-rebuttal.tex <==
\twocolumn

\noindent 
We thank the reviewers for their valuable feedback and constructive suggestions. 
%
Overall, the reviewers considered our paper well written (\textcolor{blue}{RB}, \textcolor{blue}{RC}, \textcolor{blue}{RD}), and appreciated the important and interesting target problem (\textcolor{blue}{RA}, \textcolor{blue}{RC}, \textcolor{blue}{RD}), technically soundness (\textcolor{blue}{RC}, \textcolor{blue}{RD}) as well as
extensive experiments on real MLaaS platforms (\textcolor{blue}{RA}, \textcolor{blue}{RB}, \textcolor{blue}{RC}, \textcolor{blue}{RD}).
%
The reviewers also required more justifications for the motivation of the threat model (\textcolor{blue}{RA}, \textcolor{blue}{RB}) and raised some concerns about the attack generalization (\textcolor{blue}{RA}), attack performance on larger datasets (\textcolor{blue}{RC}, \textcolor{blue}{RD}) and new countermeasures (\textcolor{blue}{RC}, \textcolor{blue}{RD}).
%
In what follows, we provide a detailed response to each reviewer's comments to address their concerns, where RiQj denotes the comment Qj from Reviewer i.
%
Note that some references in this rebuttal are the same as in the paper and thus omitted. 

\vspace{1mm}

\noindent
{\color{blue}RAQ1}. The threat model needs better justification. Typically, the explanation of the model's decision needs to be interpreted together with its corresponding input. It's unclear to me how in practice the victim would release the explanations only.


\noindent
{\color{blue}Response}. (1) The Shapley values indicate feature importance and can be presented independently as shown in Fig. 1. We have investigated the Shapley value-based studies and found that whether to include the private features in the explanation reports or not depends on the practitioners and target users. For example, QII [18], GAMI-Net [63] and the demo on Google AI Platform [16] only illustrate feature importance in explanation reports. Meanwhile, the report demos on IBM x360 [3] and SHAP library [32] include both the explanations and private features. (2) We give some examples of explanation releases. For companies, the explanations can help evaluate model bias and correctness, e.g., identify dataset shift where training data is different from test data [44], understand where the model is more or less confident as a means of improving its performance [6]. In these cases, the company needs to transmit model explanations to ML service providers (could be the third party) for analysis [6]. For customers, the explanations could be shared on social media and obtained by the adversary [ZZX+21]. Because few studies or reports have considered the privacy risks in Shapley values, both the companies and customers may underestimate the sensitivity of model explanations and transmit them in plaintext. (3) We have added these justifications in the revised paper.


\noindent [ZZX+21] Xuejun Zhao, Wencan Zhang, Xiaokui Xiao and Brian Lim. \textit{Exploiting explanations for model inversion attacks}. ICCV 2021.

\noindent
{\color{blue}RAQ2}. The results are fairly intuitive and not surprising. As the explanation is generated according to the given input, privacy leakages are fairly intuitive. It's unclear to me what new insights we can draw from the results.

\noindent
{\color{blue}Response}. We would like to highlight some of our contributions: (1) this is the first paper to consider the privacy leakage of Shapley values (RD), which is interesting (RA, RC, RD) and important (RA, RB, RD); (2) we theoretically analyze the connections between private features and Shapley values in an information-theoretic perspective, which is novel and interesting (RC); (3) The proposed attack based on linearity and generalized additive model with a bounded estimation error is novel (RC) and grounded (RD); (4) The experimental results are great (RB) and worthwhile (RD); (5) We refer the reviewer to the response of RDQ4 for more discussion on the results.

\noindent
{\color{blue}RAQ3}. The attack (especially the one with auxiliary data) is applicable to any interpretation model. I would suggest developing attacks tailored to the Shapley value-based interpretation, which can be more interesting.


\noindent
{\color{blue}Response}. We respectively disagree with this comment. Our attacks are based on the inherent limitation of Shapley values. Specifically, we can simplify the computation of Shapley value into three steps: first, use an affine transformation to generate a feature replacement dataset from $x$ and $x^0$, then feed the dataset into the model, and finally use another affine transformation on the model outputs to get Shapley values. We first observe that the mapping from private features to Shapley values is fixed, then theoretically analyze the privacy risks of Shapley values via mutual information (Eq. 13) and accordingly propose the inverse mapping attack (attack 1) and generalized additive model (GAM) transformation-based attack (attack 2). On the contrary, other popular explanation methods, e.g., LIME [44] and DeepLIFT [53], focus on approximating the linear decision boundary around the target features via a set of heuristic rules, where the mappings between features and explanations among different samples are unstable and undefined, leading to little convergence of attack 1 and invalidating the GAM transformation and error bounds of attack 2. \textcolor{red}{TODO} We thank the reviewer for this comment and have added more discussion on the attack generalization in the revised paper.

% (2) Fig. 5 shows that our attacks can achieve far better results than the baselines and indicate clear privacy leakage (RB, RD). Although simple, the proposed attacks are robust, well-grounded and performant.

\vspace{1mm}

\noindent
{\color{blue}RBQ1}. To me it is clear that the explanations include a lot of information about the example itself. Why is it reasonable to disclose these explanations to an adversary?

\noindent
{\color{blue}Response}. Please refer to the response of RAQ1.

\noindent
{\color{blue}RBQ2}. Why can't the service provider do the analysts internally? Also, what kind of useful analysis can be done without knowing the underlying example?


\noindent
{\color{blue}Response}. The service provider can choose to do the analysis internally or outsource it to ML providers. Please refer to the response of RAQ1 for examples. In addition, [31] shows that data outsourcing is common among companies via the case "Facebook and Cambridge Analytica".


\noindent
{\color{blue}RBQ3}. Does the attack work if there are multiple features missing?

\noindent
{\color{blue}Response}. Yes, attack 1 can reconstruct all the private features based on their Shapley values and an auxiliary dataset (Algorithm 1); attack 2 can also recover all the private features based on only the Shapley values (Algorithm 2) but discard some features that have large estimation errors (Eq. 21). We would like to note that feature selection and replacements happen only in the computation of Shapley values which is treated as a black box and has little relation to the attack algorithms.

\vspace{1mm}

\noindent
{\color{blue}RCQ1}. The motivation requires the explanation variable $s_i$ to be from Gaussian distribution. Is this assumption satisfied in practice? Can you verify it in your studies datasets?



\noindent
{\color{blue}Response}. (1) The Gaussian assumption of Shapley values has been analyzed in previous studies, e.g., [AOG19] and [CL21]. (2) As advised, we further conducted a $\chi^2$ goodness-of-fit test on the Shapley values generated on the Google platform from two datasets: Bank and Diabetes, where $H_0$ is "Gaussian density (theoretical) distribution can well fit the density distribution of the observed Shapley values". Test results show that for Shapley values generated from both Bank and Diabetes, the divergence statistics are 3.84 and 2.48, and $p$ values are 0.998 and 0.999. Therefore, under any significance level $\alpha$, such as $\alpha=0.05$, we can not reject $H_0$, i.e., Gaussian distribution can well fit the observed Shapley values. 

\noindent
[AOG19] Marco Ancona, Cengiz Oztireli, and Markus Gross. \textit{Explaining deep neural networks with a polynomial time algorithm for shapley value approximation}. ICML 2019.

\noindent
[CL21] Ian Covert, and Su-In Lee. \textit{Improving KernelSHAP: Practical Shapley value estimation using linear regression}. AISTATS, 2021.


\noindent
{\color{blue}RCQ2}. My another main concern is about the evaluation: 1) Dataset: The considered datasets are rather small. Is it possible to test the attack on larger datasets? 2) Metric MAE or l1-loss: It is based on absolute difference that is magnitude dependent. Why not using the relative difference, which is magnitude independent?

\noindent
{\color{blue}Response}. (1) \textcolor{red}{TODO} (2) We would like to note that in data pre-processing, all features in all datasets are normalized into the same magnitude, i.e., [0, 1], for model training and ease of comparison (Section 5.1). Thus the $\ell_1$ loss can also indicate the relative difference in our experiments.  


\noindent
{\color{blue}RCQ3}.  Baseline using Gaussian distribution (0.5, $0.25^2$) is ad-hoc. Do you have any insights about this setting?


\noindent
{\color{blue}Response}. Since all the features are normalized into [0, 1], this Gaussian distribution can generate random values falling in [0, 1] with a probability of at least $95\%$. This baseline is consistent with previous studies [33]. We have added more justification for this baseline in the revised paper.


\noindent
{\color{blue}RCQ4}. How to understand feature importance via MACC? More specifically, in what case does Equation 24 have the maximum value? Are all $\hat{y}_j$ equal?

\noindent
{\color{blue}Response}. (1) MACC measures the linear correlation between a feature $x_i$ and the model outputs. A larger MACC indicates that the change of $x_i$ can produce larger variations in the model outputs. (2) Eq. 24 achieves the maximum when the model is linear, e.g., $Y=WX+b$. (3) $\{\hat{y}_j\}^c_{j=1}$ indicate the model outputs and should sum up to 1. And whether all $\hat{y}_j$ are equal or not depends on the model outputs.

\noindent
{\color{blue}RCQ5}. In some cases, MACC is large/small, but the respective l1 loss is also large/small. For instance, Syn-75$\%$ (0.670 vs 0.066, 0.119 vs 0.040). Can you provide some clarifications about these cases?

\noindent
{\color{blue}Response}.  The reason is that the attack model may fail to accurately learn the mapping between a few features and the Shapely values since the capacity of the black-box model is larger than that of the attack model. We thank the reviewer for pointing out this issue and have added some clarifications in the revised paper.

\noindent
{\color{blue}RCQ6}. Please discuss the relation between "Wang et al., Privacy-Preserving Representation Learning on Graphs: A Mutual Information Perspective, KDD’2021" and the proposed scheme via mutual information. Can you provide discussion or make comments on whether is it possible to also use mutual information as a defense, like Wang et al.?


\noindent
{\color{blue}Response}. (1) The idea of the graph paper [WGL+21] is similar in spirit to our analysis in Section 4.1, as it also tries to preserve privacy by reducing the mutual information between the plaintext outputs and private data. However, the method in [WGL+21] has two major differences from ours. First, [WGL+21] aims to change the learning objectives via mutual information during model training, whereas the model is trained and fixed in the computation of Shapley values; Second, the mutual information for privacy preserving in [WGL+21] is loosely related to the primary task and thus can be minimized, whereas in our case, minimizing the mutual information between Shapley values and features can harm the utility of explanations. (2) Nevertheless, we can reduce the mutual information between Shapley values and features to some extent to mitigate the proposed attacks as analyzed in [WGL+21] and discussed in Section 6 of our paper. (3) We have added the discussion in the revised paper.


\noindent
{\color{blue}RCQ7}. Minors: L1 loss is used in all figures. I suggest changing Equation (22) to be l1-loss. Pearson correlation is mentioned in Page 5, but is defined in Page 10.

\noindent
{\color{blue}Response}. As advised, we have changed the MAE in Eq. 22 to $\ell_1$ loss and moved the definition of Pearson correlation to page 5.

\vspace{1mm}

\noindent
{\color{blue}RDQ1}. Technical novelty of the attack is somewhat limited. The first attack basically trains a model to invert the mapping of features to Shapley values. 


\noindent
{\color{blue}Response}. We would like to refer the reviewer to the response of RAQ3 for the discussion on attack generalization.

\noindent
{\color{blue}RDQ2}. If the problem is indeed the dimension of Shapley values, then countermeasures should include ones that reduce the number of Shapley values released, like releasing only the largest k Shapley values or only releasing Shapley values above a threshold.

\noindent
{\color{blue}Response}. We thank the reviewer for this suggestion. (1) We would like to note that the variance of Shapley values, instead of the value intensity, indicates the importance of features (Eq. 13), and releasing Shapley values based on their intensities may harm the utility of explanations because the important features in some samples may have small Shapley values. Instead, we can empirically choose the top $k$ important features based on their Shapley variances and only release the Shapley values of these $k$ features as a defense.  (2) We note that releasing only $k$ Shapley values causes little impact on the accuracy of attack 2 because the features are reconstructed independently based on the corresponding Shapley values (Algorithm 2). (3) As advised, we added an experiment to test the  performance of attack 1 on Adult and Bank via 1000 queries to the Google platform, in which we only release $k$ Shapley values and recover the $k$ corresponding features. When the numbers of released Shapley values vary in $\{20\%n, 50\%n, n\}$, the averaging $\ell_1$ losses of Adult and Bank are $\{0.0824, 0.0909, 0.0905\}$ and $\{0.0546, 0.0619, 0.0643\}$, respectively. The results are consistent with our analysis: the Shapley values of more important features leak more private information (Section 4.1.1) since the models tend to build linear connections between these features and their predictions (Section 4.2.2). (4) The conclusion is that releasing only $k$ Shapley values can reduce the success rates of the proposed attacks to at most $k/n$ but impact little on the accuracy of the recovered features. (5) We have added this defense in the revised paper.


\noindent
{\color{blue}RDQ3}. The paper uses a variety of datasets but they all of them have (relatively) few classes and features. One may conjecture that the problem could get harder (or easier) with a much larger feature set.




\noindent
{\color{blue}Response}. As advised, we have added a new experiment, in which \textcolor{red}{TODO}



\noindent
{\color{blue}RDQ4}. I think it would be substantially improved if it made more effort to uncover the factors that impact attack performance. Some understanding of what kind of features for the data or what kind of target model leads to greater vulnerability would be very interesting.



\noindent
{\color{blue}Response}. (1) The results of Section 5.4 show that the important features, which have close relations with model outputs, are more vulnerable to the proposed attacks. Based on Eq. 13, we can further conclude that the variances of Shapley values corresponding to important features are larger than that of less important features. (2) From the results of Section 5.2, we conclude that in general, NN > SVM > RF > GBDT w.r.t. the vulnerability to attacks. NN is most vulnerable because the non-linear activations, e.g., ReLU and Sigmoid, can behave in very linear ways for the important features, leading to a linear correlation between features and their Shapley values. This conclusion is consistent with previous studies [GSS15]. (3) We have added this discussion in the revised paper.

\noindent
[GSS15]	Ian J. Goodfellow, Jonathon Shlens and Christian Szegedy:
\textit{Explaining and Harnessing Adversarial Examples}. ICLR 2015.














































==> tex-files/sec-revision-letter.tex <==
\onecolumn
\thispagestyle{empty}
\centerline{\textbf{\Large Summary of Changes to CCS Submission $\#$119}}
\vspace{10mm}


\noindent We would like to thank all the reviewers for the positive feedback and insightful comments.
%
In this letter, we first provide a summary of major changes.
Then, we present detailed responses to each revision criterion.
%
The changes in the revised paper are highlighted in {\color{blue} blue}.

\section*{Summary of Major Changes}
\label{sec-changes}
We have made the following major changes in this revision:

\begin{itemize}[topsep=2pt,itemsep=2mm,parsep=0pt,partopsep=0pt,leftmargin=20pt]
    \item Section~\ref{sec-intro}: we have added more clarifications of technical challenges and the motivation of the threat model, in response to \textbf{revision criterion 1} and \textbf{2}.
    \item Section~\ref{subsec-attack-1}: we have justified the Gaussian distribution assumption on Shapley values via a $\chi^2$ goodness-of-fit test, in response to \textbf{revision criterion 5}.
    \item Section~\ref{subsec-attack-generalization}: we have added more discussion to clarify the technical novelty of our attacks, in response to \textbf{revision criterion 2}.
    \item Section~\ref{sec-exp}: we have included additional experimental results with larger datasets, in response to \textbf{revision criterion 3}.
    \item Section~\ref{sec-countermeasure}: we have discussed the countermeasure via mutual information and the countermeasure pointed by reviewer D, in response to \textbf{revision criterion 4} and \textbf{6}.
    \item Section~\ref{sec-related-work}: we have added the discussion of the relation between Wang et al.'s work~\cite{wang2021privacy} and our attacks via mutual information, in response to \textbf{revision criterion 6}.
    \item Section~\ref{sec-discussion}: we have added the discussion of the impact of large datasets on attack performance, in response to \textbf{revision criterion 3}.
\end{itemize}


\section*{Response to Revision Criteria}

% \vspace{2mm}\noindent
\textbf{Criterion 1.} \textit{Clarify the motivation of the threat model. Particularly, why an adversary should have access to the explanations, or to say, a victim releases the explanations only?}

\vspace{2mm}\noindent
\textbf{Response.} We have clarified the attack motivation by including more examples of explanation releases in  Section~\ref{sec-intro} and Footnote~\ref{footnote-sep-input-exp}. 


\vspace{2mm}\noindent
\textbf{Criterion 2.} \textit{Better clarify the technical novelty and challenges}.

\vspace{2mm}\noindent
\textbf{Response.} We have added more clarifications of the technical challenges in Section~\ref{sec-intro} and new discussions of the technical novelty in Section~\ref{subsec-attack-generalization}. Specifically, in Section~\ref{subsec-attack-generalization}, we give the intuitive idea behind our algorithm designs and discuss the optimizations made for Shapley values in our attacks. We further analyze the generalization of our attacks on other popular explanation methods and give new experimental results to justify our analysis.

\vspace{2mm}\noindent
\textbf{Criterion 3.} \textit{Evaluations on large datasets (e.g., more data, classes, and features)}.

\vspace{2mm}\noindent
\textbf{Response.} We have performed attacks on two large datasets: \textit{IDA} 2016 Challenge~\cite{UCI} with 76000 instances and 170 features, \textit{Insurance} Company Benchmark~\cite{insurance} with 90000 instances and 85 features. The corresponding results are included in Fig.~\ref{fig-loss-sizes} and Tab.~\ref{tb-success-sizes-attack2}. 
% 
In addition, we have added more discussion on the impact of large datasets (i.e., more instances, classes and features) on the attack performance in Section~\ref{sec-discussion}. 


\vspace{2mm}\noindent
\textbf{Criterion 4.} \textit{Evaluations on countermeasures pointed by reviewer D}.

\vspace{2mm}\noindent
\textbf{Response.} We have added the discussion of  the countermeasure pointed by reviewer D  in Section~\ref{sec-countermeasure}. Correspondingly, we have conducted attack experiments \textit{w.r.t.} this countermeasure on the Google Cloud Platform with two real-world datasets, Adult and Bank. The results are also included in Section~\ref{sec-countermeasure}.


\vspace{2mm}\noindent
\textbf{Criterion 5.} \textit{Justify the Gaussian distribution assumption in real-world applications}.

\vspace{2mm}\noindent
\textbf{Response.} We have justified this assumption by a $\chi^2$ goodness-of-fit test on the Shapley values generated on the Google Cloud Platform from two real-world datasets: Bank and Diabetes. The test results are included in Footnote~\ref{footnote-gaussian}.



\vspace{2mm}\noindent
\textbf{Criterion 6.} \textit{Discuss the countermeasures via mutual information}.

\vspace{2mm}\noindent
\textbf{Response.} We have added the discussion of the countermeasure ``reducing the mutual Information between inputs and Shapley values'' in Section~\ref{sec-countermeasure}. In addition, we have added the discussion of the difference between the defense mechanisim in Wang et al.'s work~\cite{wang2021privacy} and the countermeasure in our paper in Section~\ref{sec-related-work}.

\vspace{2mm}\noindent
\textbf{Minor.} \textit{Minor changes}.

\vspace{2mm}\noindent
\textbf{Response.} (1) We have added the explanation for the parameter choice of the Gaussian baseline $\boldsymbol{N}(0.5,0.25^2)$ in Section~\ref{subsec-exp-setting}. 
(2) We have added the explanation for the meaning of MACC in Section~\ref{subsec-exp-feature}. 
(3) We have added the explanation for the inconsistency between the MACCs and $\ell_1$ losses of some features in Fig.~\ref{fig-per-feature}. 
(4) We have changed the ``MAE'' in Eq.~\ref{eq-l1} to $\ell_1$. 
(5) We have moved the definition of Pearson Correlation Coefficient from Section~\ref{subsec-exp-feature} to Footnote~\ref{footnote-pearson}. 
(6) We have added more discussions of the factors that impact the attack performance in Section~\ref{sec-conclusion}.


\twocolumn
